Predicting battery end of life from solar off-grid system field data using machine learning

Hundreds of millions of people lack access to electricity. Decentralised solar-battery systems are key for addressing this whilst avoiding carbon emissions and air pollution, but are hindered by relatively high costs and rural locations that inhibit timely preventative maintenance. Accurate diagnosis of battery health and prediction of end of life from operational data improves user experience and reduces costs. But lack of controlled validation tests and variable data quality mean existing lab-based techniques fail to work. We apply a scaleable probabilistic machine learning approach to diagnose health in 1027 solar-connected lead-acid batteries, each running for 400-760 days, totalling 620 million data rows. We demonstrate 73% accurate prediction of end of life, eight weeks in advance, rising to 82% at the point of failure. This work highlights the opportunity to estimate health from existing measurements using `big data' techniques, without additional equipment, extending lifetime and improving performance in real-world applications.

==> Tables/1_Week_ahead_perf_summary.tex <==
\begin{tabular}{llllll}
\toprule
I (\SI{}{\ampere}) & T (\SI{}{\kelvin}) & $\hat{c}$ (\SI{}{\mole\per\meter\cubed}) & Precision (\%) & Recall (\%) & Balanced Accuracy (\%) \\
\midrule
              0.79 &              300.2 &                                     4338 &           79.6 &        57.5 &                   73.6 \\
              0.79 &              296.7 &                                     4338 &           78.4 &        58.1 &                   73.4 \\
              0.58 &              296.7 &                                     4338 &           78.3 &        55.9 &                   72.4 \\
              0.58 &              300.2 &                                     4338 &           77.1 &        56.1 &                   72.1 \\
              0.79 &              296.7 &                                     4730 &           78.6 &        54.5 &                     72 \\
              0.79 &              300.2 &                                     4730 &           76.9 &        54.1 &                   71.3 \\
              0.79 &              303.7 &                                     4730 &           76.3 &          53 &                   70.6 \\
              1.01 &              303.7 &                                     4730 &           73.5 &        53.6 &                     70 \\
              0.58 &              296.7 &                                     4730 &           76.5 &        50.2 &                   69.5 \\
              0.58 &              300.2 &                                     4730 &           74.9 &        49.5 &                   68.8 \\
              0.79 &              300.2 &                                     5121 &           75.2 &        48.2 &                   68.3 \\
              1.01 &              300.2 &                                     4730 &             72 &          50 &                   68.1 \\
              0.79 &              303.7 &                                     5121 &           74.2 &          48 &                   67.9 \\
              1.01 &              303.7 &                                     5121 &           70.7 &        50.2 &                   67.8 \\
         $I^\mu_i$ &          $T^\mu_i$ &                          $\hat{c}^\mu_i$ &           74.8 &        46.4 &                   67.4 \\
              1.01 &              300.2 &                                     5121 &           68.2 &          47 &                   65.6 \\
\bottomrule
\end{tabular}


==> Tables/Class_hypers.tex <==
\begin{tabular}{rrrrrrrrrrrr}
\toprule
 Horizon &  $\sigma^2_\mathrm{f}$ &  R$_0$ &  $\partial$R$_0$/$\partial$t &  Age &  $\Sigma$ Ah &  $\Sigma$ cyc &  $\Sigma$  t$_\mathrm{float}$ &  $\Sigma$  t$_\mathrm{low V}$ &  $\Sigma$ t$_\mathrm{high V}$ &  $\Sigma$ t$_\mathrm{low T}$ &  $\Sigma$ t$_\mathrm{high T}$ \\
\midrule
           0 &                   3.54 &   1.23 &                         1.14 & 0.42 &         3.14 &          8.78 &                          7.22 &                          2.16 &                          7.44 &                         3.50 &                          2.99 \\
           2 &                   3.87 &   1.48 &                         3.24 & 0.49 &         3.57 &          4.59 &                          4.84 &                          2.29 &                         10.74 &                         4.64 &                          2.87 \\
           4 &                   3.99 &   1.33 &                         4.37 & 0.33 &         3.78 &          4.54 &                          5.51 &                          2.32 &                          9.63 &                         4.12 &                          3.22 \\
           6 &                   3.73 &   1.47 &                         1.96 & 0.31 &         1.74 &          3.12 &                          4.79 &                          2.95 &                          7.81 &                         3.65 &                          1.02 \\
           8 &                   3.57 &   1.26 &                         2.39 & 0.18 &         1.53 &          2.96 &                          6.88 &                          2.89 &                          6.62 &                         2.37 &                          1.30 \\
\bottomrule
\end{tabular}


==> Tables/Class_hypers_8.tex <==
\begin{tabular}{rrrrrrrrrr}
\toprule
 $\sigma_f^2$ &     R &  dR/dt &   Age &  Time$_\text{float}$ &  Time$_\text{low V}$ &  Cycle count &  Time$_\text{high T}$ &  Total Ah &  Time$_\text{high V}$ \\
\midrule
        3.151 & 1.426 &  1.739 & 0.617 &                9.589 &                 2.23 &        1.983 &                 1.121 &     1.483 &                 1.739 \\
\bottomrule
\end{tabular}


==> Tables/Class_hypers_diag_P.tex <==
\begin{tabular}{rrrrrrrrrrrr}
\toprule
 Weeks ahead &  $\sigma^2_\mathrm{f}$ &  R$_0$ &  $\partial$R$_0$/$\partial$t &  Age &  $\Sigma$ Ah &  $\Sigma$ cyc &  $\Sigma$  t$_\mathrm{float}$ &  $\Sigma$  t$_\mathrm{low V}$ &  $\Sigma$ t$_\mathrm{high V}$ &  $\Sigma$ t$_\mathrm{low T}$ &  $\Sigma$ t$_\mathrm{high T}$ \\
\midrule
           0 &                   3.90 &   1.02 &                         1.63 & 0.46 &         1.97 &          5.97 &                          5.85 &                          2.28 &                          6.49 &                         2.70 &                          1.40 \\
           2 &                   3.91 &   1.13 &                         4.45 & 0.61 &         1.97 &          5.23 &                          5.63 &                          2.38 &                         10.47 &                         4.63 &                          5.16 \\
           4 &                   4.13 &   1.34 &                         2.41 & 0.42 &         2.07 &          2.93 &                          2.93 &                          2.48 &                          9.53 &                         2.35 &                          1.09 \\
           6 &                   3.85 &   1.69 &                         2.04 & 0.33 &         1.73 &          3.16 &                          7.72 &                          2.44 &                          6.77 &                         2.22 &                          1.19 \\
           8 &                   4.09 &   1.51 &                         2.54 & 0.35 &         1.94 &          2.76 &                          9.85 &                          3.05 &                          7.37 &                         2.80 &                          1.45 \\
\bottomrule
\end{tabular}


==> Tables/Class_result_3w_cutoff.tex <==
\begin{table}
\centering

\begin{tabular}{llllll}
\toprule
I (\SI{}{\ampere}) & T (\SI{}{\kelvin}) & $\hat{c}$ (\SI{}{\mole\per\meter\cubed}) & Precision (\%) & Recall (\%) & Balanced Accuracy (\%) \\
\midrule
              0.78 &              300.1 &                                     4370 &           75.1 &        54.4 &                   71.4 \\
              0.57 &              300.1 &                                     4370 &           74.6 &        54.5 &                   71.4 \\
              0.57 &              296.5 &                                     4370 &           74.9 &        52.9 &                     71 \\
              0.78 &              296.5 &                                     4370 &           73.8 &        50.3 &                   69.6 \\
              0.57 &              300.1 &                                     4747 &           74.2 &        46.6 &                   68.3 \\
              0.99 &              300.1 &                                     4747 &           72.5 &        47.5 &                   68.1 \\
         $I^\mu_i$ &          $T^\mu_i$ &                          $\hat{c}^\mu_i$ &             73 &        46.5 &                   67.8 \\
              0.78 &              300.1 &                                     4747 &           71.5 &        46.7 &                   67.6 \\
              0.78 &              296.5 &                                     4747 &           71.4 &          47 &                   67.6 \\
              0.57 &              296.5 &                                     4747 &             72 &        46.1 &                   67.2 \\
              0.78 &              303.6 &                                     4747 &           70.7 &        45.7 &                   66.8 \\
              0.99 &              303.6 &                                     4747 &           70.2 &        44.3 &                   66.2 \\
              0.99 &              300.1 &                                     5124 &           74.2 &        40.8 &                   65.9 \\
              0.78 &              303.6 &                                     5124 &           68.7 &        44.4 &                   65.8 \\
              0.99 &              303.6 &                                     5124 &           68.5 &          44 &                   65.6 \\
              0.78 &              300.1 &                                     5124 &           71.8 &        39.7 &                   64.9 \\
\bottomrule
\end{tabular}

\caption{Average test-set classification performance for 5-fold cross validation at different operating points.($(I^\mu_i,T^\mu_i,\hat{c}^\mu_i$) denotes the batterywise mean operating point.}
\label{tbl:class_perf}
\end{table}


==> Tables/Hypers_medians.tex <==
\begin{tabular}{rrrrrr}
\toprule
 Weeks before &  $l_\mathrm{T}$ &  $l_\mathrm{I}$ &  $l_\mathrm{\hat{c}}$ &  $\sigma_\mathrm{f,0}$ &  $\sigma_\mathrm{f,1}$ \\
\midrule
            0 &            3.51 &            1.70 &                  2.78 &                   0.96 &                   0.31 \\
           14 &            3.72 &            1.71 &                  2.80 &                   0.94 &                   0.31 \\
           28 &            3.79 &            1.71 &                  2.83 &                   0.89 &                   0.31 \\
           42 &            3.72 &            1.70 &                  2.86 &                   0.89 &                   0.31 \\
           56 &            3.70 &            1.71 &                  2.86 &                   0.83 &                   0.31 \\
\bottomrule
\end{tabular}


==> Tables/Hypers_medians_diag_P.tex <==
\begin{tabular}{rrrrrr}
\toprule
 Weeks before &  $l_\mathrm{T}$ &  $l_\mathrm{I}$ &  $l_\mathrm{\hat{c}}$ &  $\sigma_\mathrm{f,0}$ &  $\sigma_\mathrm{f,1}$ \\
\midrule
            0 &            2.28 &            1.91 &                  2.06 &                   0.98 &                   0.25 \\
           14 &            2.27 &            1.93 &                  2.16 &                   0.98 &                   0.25 \\
           28 &            2.35 &            1.97 &                  2.16 &                   0.97 &                   0.25 \\
           42 &            2.33 &            1.93 &                  2.13 &                   0.96 &                   0.25 \\
           56 &            2.33 &            1.97 &                  2.12 &                   0.96 &                   0.25 \\
\bottomrule
\end{tabular}


==> Tables/Perf_long_table_all_fac_bayes_factor.tex <==
\begin{tabular}{rlrrrrrr}
\toprule
 Days before &                                   Classifier input &  TP &  FP &  FN &  TN &  Balanced Accuracy (\%) &  Bayes Factor \\
\midrule
           0 &                                        R benchmark & 221 &  82 & 243 & 571 &                    67.5 &           3.8 \\
           0 &                 R, $\frac{\partial R}{\partial t}$ & 309 &  85 & 155 & 568 &                    76.8 &           5.1 \\
           0 & R, $\frac{\partial R}{\partial t}$, stress factors & 370 &  56 &  94 & 597 &                    85.6 &           9.3 \\
          14 &                                        R benchmark & 161 &  75 & 303 & 578 &                    61.6 &           3.0 \\
          14 &                 R, $\frac{\partial R}{\partial t}$ & 261 &  82 & 203 & 571 &                    71.8 &           4.5 \\
          14 & R, $\frac{\partial R}{\partial t}$, stress factors & 359 &  57 & 105 & 596 &                    84.3 &           8.9 \\
          28 &                                        R benchmark & 126 &  60 & 338 & 593 &                    59.0 &           3.0 \\
          28 &                 R, $\frac{\partial R}{\partial t}$ & 241 &  85 & 223 & 568 &                    69.5 &           4.0 \\
          28 & R, $\frac{\partial R}{\partial t}$, stress factors & 336 &  62 & 128 & 591 &                    81.5 &           7.6 \\
          42 &                                        R benchmark & 104 &  49 & 360 & 604 &                    57.5 &           3.0 \\
          42 &                 R, $\frac{\partial R}{\partial t}$ & 209 &  87 & 255 & 566 &                    65.9 &           3.4 \\
          42 & R, $\frac{\partial R}{\partial t}$, stress factors & 355 &  65 & 109 & 588 &                    83.3 &           7.7 \\
          56 &                                        R benchmark &  75 &  63 & 389 & 590 &                    53.3 &           1.7 \\
          56 &                 R, $\frac{\partial R}{\partial t}$ & 172 &  92 & 292 & 561 &                    61.5 &           2.6 \\
          56 & R, $\frac{\partial R}{\partial t}$, stress factors & 333 &  77 & 131 & 576 &                    80.0 &           6.1 \\
\bottomrule
\end{tabular}


==> Tables/Perf_long_table_all_fac_bayes_factor_diag_P.tex <==
\begin{tabular}{rlrrrrrr}
\toprule
 Days before &                                   Classifier input &  TP &  FP &  FN &  TN &  Balanced Accuracy (\%) &  Bayes Factor \\
\midrule
           0 &                                        R benchmark & 221 &  82 & 243 & 571 &                    67.5 &           3.8 \\
           0 &                 R, $\frac{\partial R}{\partial t}$ & 304 &  68 & 160 & 585 &                    77.6 &           6.3 \\
           0 & R, $\frac{\partial R}{\partial t}$, stress factors & 381 &  46 &  83 & 607 &                    87.5 &          11.7 \\
          14 &                                        R benchmark & 161 &  75 & 303 & 578 &                    61.6 &           3.0 \\
          14 &                 R, $\frac{\partial R}{\partial t}$ & 253 &  74 & 211 & 579 &                    71.6 &           4.8 \\
          14 & R, $\frac{\partial R}{\partial t}$, stress factors & 356 &  59 & 108 & 594 &                    83.8 &           8.5 \\
          28 &                                        R benchmark & 126 &  60 & 338 & 593 &                    59.0 &           3.0 \\
          28 &                 R, $\frac{\partial R}{\partial t}$ & 231 &  74 & 233 & 579 &                    69.2 &           4.4 \\
          28 & R, $\frac{\partial R}{\partial t}$, stress factors & 355 &  61 & 109 & 592 &                    83.6 &           8.2 \\
          42 &                                        R benchmark & 104 &  49 & 360 & 604 &                    57.5 &           3.0 \\
          42 &                 R, $\frac{\partial R}{\partial t}$ & 195 &  75 & 269 & 578 &                    65.3 &           3.7 \\
          42 & R, $\frac{\partial R}{\partial t}$, stress factors & 353 &  74 & 111 & 579 &                    82.4 &           6.7 \\
          56 &                                        R benchmark &  75 &  63 & 389 & 590 &                    53.3 &           1.7 \\
          56 &                 R, $\frac{\partial R}{\partial t}$ & 175 &  84 & 289 & 569 &                    62.4 &           2.9 \\
          56 & R, $\frac{\partial R}{\partial t}$, stress factors & 340 &  77 & 124 & 576 &                    80.7 &           6.2 \\
\bottomrule
\end{tabular}


==> Tables/Perf_long_table_all_fac_diag_P.tex <==
\begin{tabular}{rlrrrrr}
\toprule
 Days before &                                   Classifier input &  TP &  FP &  FN &  TN &  Balanced Accuracy (\%) \\
\midrule
           0 &                                          Benchmark & 218 &  81 & 246 & 572 &                    67.3 \\
           0 &                 R, $\frac{\partial R}{\partial t}$ & 304 &  79 & 160 & 574 &                    76.7 \\
           0 & R, $\frac{\partial R}{\partial t}$, stress factors & 381 &  58 &  82 & 595 &                    86.7 \\
           0 &                                Stress factors only & 326 &  73 & 138 & 580 &                    79.5 \\
          14 &                                          Benchmark & 158 &  73 & 306 & 580 &                    61.4 \\
          14 &                 R, $\frac{\partial R}{\partial t}$ & 278 &  77 & 186 & 576 &                    74.1 \\
          14 & R, $\frac{\partial R}{\partial t}$, stress factors & 370 &  71 &  93 & 582 &                    84.5 \\
          14 &                                Stress factors only & 331 &  72 & 133 & 581 &                    80.2 \\
          28 &                                Stress factors only & 333 &  75 & 131 & 578 &                    80.1 \\
          28 & R, $\frac{\partial R}{\partial t}$, stress factors & 358 &  74 & 105 & 579 &                    83.0 \\
          28 &                 R, $\frac{\partial R}{\partial t}$ & 232 &  86 & 232 & 567 &                    68.4 \\
          28 &                                          Benchmark & 126 &  60 & 338 & 593 &                    59.0 \\
          42 &                                          Benchmark & 104 &  51 & 360 & 602 &                    57.3 \\
          42 &                 R, $\frac{\partial R}{\partial t}$ & 212 &  81 & 252 & 572 &                    66.6 \\
          42 & R, $\frac{\partial R}{\partial t}$, stress factors & 358 &  76 & 105 & 577 &                    82.8 \\
          42 &                                Stress factors only & 332 &  76 & 132 & 577 &                    80.0 \\
          56 &                                          Benchmark &  67 &  56 & 397 & 597 &                    52.9 \\
          56 &                 R, $\frac{\partial R}{\partial t}$ & 204 & 106 & 259 & 547 &                    63.9 \\
          56 & R, $\frac{\partial R}{\partial t}$, stress factors & 343 &  83 & 120 & 570 &                    80.7 \\
          56 &                                Stress factors only & 330 &  74 & 134 & 579 &                    79.9 \\
\bottomrule
\end{tabular}


==> Tables/Perf_short_table_all_fac_bayes_factor.tex <==
\begin{tabular}{rrrrrrr}
\toprule
 Days before &  TP &  FP &  FN &  TN &  Balanced Accuracy (\%) &  Bayes Factor \\
\midrule
           0 & 370 &  56 &  94 & 597 &                    85.6 &           9.3 \\
          14 & 359 &  57 & 105 & 596 &                    84.3 &           8.9 \\
          28 & 336 &  62 & 128 & 591 &                    81.5 &           7.6 \\
          42 & 355 &  65 & 109 & 588 &                    83.3 &           7.7 \\
          56 & 333 &  77 & 131 & 576 &                    80.0 &           6.1 \\
\bottomrule
\end{tabular}


==> Tables/Perf_short_table_all_fac_bayes_factor_diag_P.tex <==
\begin{tabular}{rrrrrrr}
\toprule
 Days before &  TP &  FP &  FN &  TN &  Balanced Accuracy (\%) &  Bayes Factor \\
\midrule
           0 & 381 &  46 &  83 & 607 &                    87.5 &          11.7 \\
          14 & 356 &  59 & 108 & 594 &                    83.8 &           8.5 \\
          28 & 355 &  61 & 109 & 592 &                    83.6 &           8.2 \\
          42 & 353 &  74 & 111 & 579 &                    82.4 &           6.7 \\
          56 & 340 &  77 & 124 & 576 &                    80.7 &           6.2 \\
\bottomrule
\end{tabular}


==> Tables/Perf_table.tex <==
\begin{tabular}{rrrrrrr}
\toprule
 Days before &   TP &  FP &   FN &   TN &  Balanced Accuracy (\%) &  MCC (\%) \\
\midrule
           0 &  299 &  66 &  165 &  587 &                    77.2 &      57.1 \\
           7 &  279 &  65 &  185 &  588 &                    75.1 &      53.7 \\
          14 &  268 &  73 &  196 &  580 &                    73.3 &      50.1 \\
          21 &  269 &  83 &  195 &  570 &                    72.6 &      48.0 \\
\bottomrule
\end{tabular}


==> Tables/Perf_table_all_fac.tex <==
\begin{tabular}{rrrrrrr}
\toprule
 Days before &  TP &  FP &  FN &  TN &  Balanced Accuracy (\%) &  MCC (\%) \\
\midrule
           0 & 374 &  51 &  90 & 602 &                    86.4 &      73.9 \\
          14 & 367 &  60 &  97 & 593 &                    85.0 &      70.9 \\
          28 & 357 &  68 & 107 & 585 &                    83.3 &      67.7 \\
          42 & 341 &  67 & 123 & 586 &                    81.6 &      64.8 \\
          56 & 335 &  72 & 129 & 581 &                    80.6 &      62.7 \\
\bottomrule
\end{tabular}


==> Tables/Weekly_perf_summary.tex <==
\begin{tabular}{rllllll}
\toprule
 Weeks before & I (\SI{}{\ampere}) & T (\SI{}{\kelvin}) & $\hat{c}$ (\SI{}{\mole\per\meter\cubed}) & Precision (\%) & Recall (\%) & Balanced Accuracy (\%) \\
\midrule
            0 &               0.79 &              296.7 &                                     4338 &           78.6 &        58.2 &                   73.5 \\
            1 &               0.79 &              300.2 &                                     4338 &           79.6 &        57.5 &                   73.6 \\
            2 &               0.79 &              300.2 &                                     4338 &           78.9 &        53.5 &                   71.6 \\
            3 &               0.79 &              296.7 &                                     4338 &           77.6 &        53.3 &                   71.2 \\
\bottomrule
\end{tabular}


==> Tables/classperf_table.tex <==
\begin{tabular}{rlrrrrr}
\toprule
 Days before &                                   Classifier input &  TP &  FP &  FN &  TN &  Balanced Accuracy (\%) \\
\midrule
           0 &                 R, $\frac{\partial R}{\partial t}$ & 339 &  77 & 152 & 459 &                    77.3 \\
           0 & R, $\frac{\partial R}{\partial t}$, stress factors & 389 &  77 & 102 & 459 &                    82.4 \\
           0 &                                          Benchmark & 244 &  95 & 247 & 441 &                    66.0 \\
           0 &                                Stress factors only & 313 & 120 & 178 & 416 &                    70.7 \\
          14 &                 R, $\frac{\partial R}{\partial t}$ & 308 &  87 & 183 & 449 &                    73.2 \\
          14 & R, $\frac{\partial R}{\partial t}$, stress factors & 378 &  88 & 113 & 448 &                    80.3 \\
          14 &                                          Benchmark & 203 &  90 & 288 & 446 &                    62.3 \\
          14 &                                Stress factors only & 336 & 139 & 155 & 397 &                    71.2 \\
          28 &                                Stress factors only & 346 & 154 & 145 & 382 &                    70.9 \\
          28 &                                          Benchmark & 170 & 126 & 321 & 410 &                    55.6 \\
          28 & R, $\frac{\partial R}{\partial t}$, stress factors & 373 & 126 & 118 & 410 &                    76.2 \\
          28 &                 R, $\frac{\partial R}{\partial t}$ & 276 & 113 & 215 & 423 &                    67.6 \\
          42 &                 R, $\frac{\partial R}{\partial t}$ & 258 & 114 & 233 & 422 &                    65.6 \\
          42 & R, $\frac{\partial R}{\partial t}$, stress factors & 367 & 135 & 124 & 401 &                    74.8 \\
          42 &                                          Benchmark & 124 & 125 & 367 & 411 &                    51.0 \\
          42 &                                Stress factors only & 353 & 181 & 138 & 355 &                    69.1 \\
          56 &                 R, $\frac{\partial R}{\partial t}$ & 245 & 127 & 246 & 409 &                    63.1 \\
          56 & R, $\frac{\partial R}{\partial t}$, stress factors & 368 & 155 & 123 & 381 &                    73.0 \\
          56 &                                          Benchmark & 107 & 109 & 384 & 427 &                    50.7 \\
          56 &                                Stress factors only & 357 & 214 & 134 & 322 &                    66.4 \\
\bottomrule
\end{tabular}


==> Tables/corr_mat.tex <==
\begin{tabular}{lrrrrrrrrrr}
\toprule
{} &  R$_0$ &  $\partial$R$_0$/$\partial$t &   Age &  $\Sigma$ Ah &  $\Sigma$ cyc &  $\Sigma$  t$_\mathrm{float}$ &  $\Sigma$  t$_\mathrm{low V}$ &  $\Sigma$ t$_\mathrm{high V}$ &  $\Sigma$ t$_\mathrm{low T}$ &  $\Sigma$ t$_\mathrm{high T}$ \\
\midrule
R$_0$                        &   1.00 &                         0.75 &  0.25 &         0.03 &          0.18 &                          0.07 &                          0.13 &                          0.04 &                         0.15 &                         -0.15 \\
$\partial$R$_0$/$\partial$t  &   0.75 &                         1.00 &  0.14 &         0.25 &          0.17 &                         -0.06 &                          0.06 &                          0.04 &                        -0.01 &                          0.01 \\
Age                          &   0.25 &                         0.14 &  1.00 &         0.29 &          0.42 &                          0.29 &                          0.05 &                          0.37 &                         0.17 &                         -0.04 \\
$\Sigma$ Ah                  &   0.03 &                         0.25 &  0.29 &         1.00 &          0.36 &                         -0.33 &                          0.11 &                          0.33 &                        -0.25 &                          0.34 \\
$\Sigma$ cyc                 &   0.18 &                         0.17 &  0.42 &         0.36 &          1.00 &                         -0.17 &                          0.00 &                         -0.05 &                         0.28 &                         -0.22 \\
$\Sigma$  t$_\mathrm{float}$ &   0.07 &                        -0.06 &  0.29 &        -0.33 &         -0.17 &                          1.00 &                         -0.17 &                          0.21 &                        -0.36 &                          0.02 \\
$\Sigma$  t$_\mathrm{low V}$ &   0.13 &                         0.06 &  0.05 &         0.11 &          0.00 &                         -0.17 &                          1.00 &                         -0.10 &                         0.00 &                         -0.05 \\
$\Sigma$ t$_\mathrm{high V}$ &   0.04 &                         0.04 &  0.37 &         0.33 &         -0.05 &                          0.21 &                         -0.10 &                          1.00 &                        -0.24 &                          0.36 \\
$\Sigma$ t$_\mathrm{low T}$  &   0.15 &                        -0.01 &  0.17 &        -0.25 &          0.28 &                         -0.36 &                          0.00 &                         -0.24 &                         1.00 &                         -0.68 \\
$\Sigma$ t$_\mathrm{high T}$ &  -0.15 &                         0.01 & -0.04 &         0.34 &         -0.22 &                          0.02 &                         -0.05 &                          0.36 &                        -0.68 &                          1.00 \\
\bottomrule
\end{tabular}


==> Tables/corr_mat_diag_P.tex <==
\begin{tabular}{lrrrrrrrrrr}
\toprule
{} &  R$_0$ &  $\partial$R$_0$/$\partial$t &   Age &  $\Sigma$ Ah &  $\Sigma$ cyc &  $\Sigma$  t$_\mathrm{float}$ &  $\Sigma$  t$_\mathrm{low V}$ &  $\Sigma$ t$_\mathrm{high V}$ &  $\Sigma$ t$_\mathrm{low T}$ &  $\Sigma$ t$_\mathrm{high T}$ \\
\midrule
R$_0$                        &   1.00 &                         0.75 &  0.27 &        -0.00 &          0.18 &                          0.11 &                          0.11 &                          0.05 &                         0.14 &                         -0.14 \\
$\partial$R$_0$/$\partial$t  &   0.75 &                         1.00 &  0.16 &         0.24 &          0.19 &                         -0.03 &                          0.07 &                          0.04 &                         0.00 &                          0.00 \\
Age                          &   0.27 &                         0.16 &  1.00 &         0.29 &          0.42 &                          0.29 &                          0.05 &                          0.37 &                         0.17 &                         -0.04 \\
$\Sigma$ Ah                  &  -0.00 &                         0.24 &  0.29 &         1.00 &          0.36 &                         -0.33 &                          0.11 &                          0.33 &                        -0.25 &                          0.34 \\
$\Sigma$ cyc                 &   0.18 &                         0.19 &  0.42 &         0.36 &          1.00 &                         -0.17 &                          0.00 &                         -0.05 &                         0.28 &                         -0.22 \\
$\Sigma$  t$_\mathrm{float}$ &   0.11 &                        -0.03 &  0.29 &        -0.33 &         -0.17 &                          1.00 &                         -0.17 &                          0.21 &                        -0.36 &                          0.02 \\
$\Sigma$  t$_\mathrm{low V}$ &   0.11 &                         0.07 &  0.05 &         0.11 &          0.00 &                         -0.17 &                          1.00 &                         -0.10 &                         0.00 &                         -0.05 \\
$\Sigma$ t$_\mathrm{high V}$ &   0.05 &                         0.04 &  0.37 &         0.33 &         -0.05 &                          0.21 &                         -0.10 &                          1.00 &                        -0.24 &                          0.36 \\
$\Sigma$ t$_\mathrm{low T}$  &   0.14 &                         0.00 &  0.17 &        -0.25 &          0.28 &                         -0.36 &                          0.00 &                         -0.24 &                         1.00 &                         -0.68 \\
$\Sigma$ t$_\mathrm{high T}$ &  -0.14 &                         0.00 & -0.04 &         0.34 &         -0.22 &                          0.02 &                         -0.05 &                          0.36 &                        -0.68 &                          1.00 \\
\bottomrule
\end{tabular}


==> Tables/hypers.tex <==
\begin{tabular}{rrrrrr}
\toprule
 Data cut off (Weeks) &  $l_\text{T}$ &  $l_\text{I}$ &  $l_\mathrm{\hat{c}}$ &  $\sigma^2_\text{f,1}$ &  $\sigma^2_\text{f,0}$ \\
\midrule
                    0 &         1.971 &         2.269 &                 2.143 &                  0.071 &                  0.574 \\
                    2 &         2.004 &         2.218 &                 2.153 &                  0.065 &                  0.551 \\
                    4 &         2.586 &         2.439 &                 2.573 &                  0.089 &                  0.876 \\
                    6 &         2.179 &         2.464 &                 2.358 &                  0.073 &                  0.581 \\
                    8 &         2.135 &         2.445 &                 2.319 &                  0.071 &                  0.578 \\
\bottomrule
\end{tabular}


==> Tables/hypers_gpr_accordeon.tex <==
\begin{tabular}{rrrrrr}
\toprule
 Data cutoff (weeks) &  l$_\mathrm{T}$ &  l$_\mathrm{I}$ &  l$_\mathrm{\hat{c}}$ &  $\sigma^2_\mathrm{f,1}$ &  $\sigma^2_\mathrm{f,0}$ \\
\midrule
                   0 &        1.553774 &        1.556085 &              1.552315 &                 0.058943 &                 1.008148 \\
                   2 &        1.582926 &        1.573297 &              1.581924 &                 0.055969 &                 1.006008 \\
                   4 &        1.568309 &        1.561432 &              1.568858 &                 0.055251 &                 1.006513 \\
                   6 &        1.584197 &        1.575289 &              1.584070 &                 0.054201 &                 1.005324 \\
                   8 &        1.570386 &        1.565376 &              1.571285 &                 0.058242 &                 1.006009 \\
\bottomrule
\end{tabular}


==> Tables/pop_stats.tex <==
\begin{tabular}{lllrrr}
\toprule
I (\SI{}{\ampere}) & T (\SI{}{\kelvin}) & $\mathrm{\hat{c}}$ (\SI{}{\mole\per\metre\cubed}) &  $\mu$\textsubscript{pop}(R\textsubscript{0}) ($\Omega$) &  $\sigma$\textsubscript{pop}(R\textsubscript{0}) ($\Omega$) &  $\bar{\sigma_i}^{-2}$(R\textsubscript{0}) ($\Omega$) \\
\midrule
              0.96 &              301.0 &                                              4678 &                                               0.57 &                                              0.137 &                                             1898.0 \\
       $\bar{I_i}$ &        $\bar{T_i}$ &                                 $\bar{\hat{c}_i}$ &                                               0.64 &                                              0.198 &                                             7131.0 \\
\bottomrule
\end{tabular}


==> Tables/pop_stats_diag_P.tex <==
\begin{tabular}{lllrrr}
\toprule
I (\SI{}{\ampere}) & T (\SI{}{\kelvin}) & $\mathrm{\hat{c}}$ (\SI{}{\mole\per\metre\cubed}) &  $\mu$\textsubscript{pop}(R\textsubscript{0}) ($\Omega$) &  $\sigma$\textsubscript{pop}(R\textsubscript{0}) ($\Omega$) &  $\bar{\sigma_i}^{-2}$(R\textsubscript{0}) ($\Omega$) \\
\midrule
              0.96 &              301.0 &                                              4678 &                                               0.56 &                                              0.122 &                                              502.0 \\
       $\bar{I_i}$ &        $\bar{T_i}$ &                                 $\bar{\hat{c}_i}$ &                                               0.64 &                                              0.186 &                                              923.0 \\
\bottomrule
\end{tabular}

